Decentralized Safe Reinforcement Learning for Voltage Control

Inverter-based distributed energy resources provide the possibility for fast time-scale voltage control by quickly adjusting their reactive power. The power-electronic interfaces allow these resources to realize almost arbitrary control law, but designing these decentralized controllers is nontrivial. Reinforcement learning (RL) approaches are becoming increasingly popular to search for policy parameterized by neural networks. It is difficult, however, to enforce that the learned controllers are safe, in the sense that they may introduce instabilities into the system. This paper proposes a safe learning approach for voltage control. We prove that the system is guaranteed to be exponentially stable if each controller satisfies certain Lipschitz constraints. The set of Lipschitz bound is optimized to enlarge the search space for neural network controllers. We explicitly engineer the structure of neural network controllers such that they satisfy the Lipschitz constraints by design. A decentralized RL framework is constructed to train local neural network controller at each bus in a model-free setting.

==> learning_linear.tex <==

% We explicitly derive the necessary and sufficient condition for a stabilizing controller in Theorem~\ref{theorem:Stable}. 
Learning is a promising way to find the optimal controllers. Unlike other results in distributed control where the topology of the stabilizing controllers is complicated, we can explicitly characterize the set of stable diagonal $\bm{K}$.
% Next theorem characterizes the set for stabilizing controllers.
% The convexity property guarantees that updating the linear coefficient with gradient descent will converge to the global optimum.  
% Define safety set as the set of stabilizing $\bm{K}$. 
% We prove that the safety set is convex and the controller obtained from RL is guaranteed to be stabilizing by projecting the learned coefficient to the safety set. 
\begin{theorem}\label{theorem:Stable}
The set of stabilizing controllers is diagonal matrix K satisfying $0\prec\bm{K}\prec 2\bm{X^{-1}}$.
\end{theorem}
% \textit{Safe learning with RNN-based framework: }
% Based on the stability condition in Theorem~\ref{theorem:Stable}, 


In general, the set of controllers has complicated topology which may not be connected~\cite{bu2019lqr}. 
Using the property of X, we show that the set is convex and can be easily characterized. 
In general, the cost function is quadratic in the state variables but it doesn’t imply convexity of the controller. 
However, here, we show
% gradient dominant with respect to the control coefficient matrix $\bm{K}$. 
the gradient update within the convex set will converge to the global optimum controller. 

In the paper, we show how the gradient update can be done online using the local measurements. 
We will present the proof for the theorem and show the extended result to more general functions. 





% We propose a safe learning approach that projects the learned coefficient matrix at each step back to the closest point in the safety set. This way, we guarantee that the learned linear controller is stabilizing. To facility efficient gradient calculations, we use a RNN based framework to integrate the state transition dynamics implicitly.  



% In our full paper, we will  show that the algorithm still have good convergence property for other cost function defined with $L_1$ norm on $\bm{V}_t$ and $\bm{q}_t$.











% Furthermore, we prove the convexity of the voltage optimization~\eqref{eq:Optimization} for quadratic cost function, which guarantees that updating the linear coefficient with gradient descent will converge to the global optimum. 
% \begin{theorem}\label{theorem:Convex}
% The optimal voltage regulation problem~\eqref{eq:Optimization} with quadratic cost function is convex with respect to $\bm{A}$.
% \end{theorem}


% Based on the stability condition in Theorem~\ref{theorem:Stable}, we propose a safe learning approach that projects the learned coefficient matrix $\hat{\bm{A}}$ at each step back to the closest point in the set of stabilizing controller as follows
% \begin{subequations}\label{eq:Projection}
% \begin{align}
% \min_{\bm{K}}\quad & ||\bm{K}-\hat{\bm{K}}||_2\label{subeq:Projection_obj}\\
% \mbox{s.t. } & 0\prec\bm{K}\prec 2\bm{X^{-1}} \label{subeq:Projection_stability}\\
% &\bm{K} \text{ is diagnal}\label{subeq:Projection_diag}
% \end{align}
% \end{subequations}
% where $\bm{K}$ is the projected coefficient matrix that satisfies the stability constraint. 




% \textit{RNN-based framework for efficient learning: } To facility efficient gradient calculations, we use a recurrent neural network (RNN) based framework to integrate the state transition dynamics \eqref{subeq:Optimization_q}-\eqref{subeq:Optimization_V} implicitly. Constraint \eqref{subeq:Optimization_bound} is satisfied by directly bounding the controller and \eqref{subeq:Optimization_stability} is satisfied by the safe RL Projection~\eqref{eq:Projection}. 
% Consequently, we eliminate all the explicit constraint~\eqref{subeq:Optimization_q}-\eqref{subeq:Optimization_stability}. The linear coefficient can be efficiently updated by gradient descent through the objective function~\eqref{subeq:Optimization_obj} with auto-differentiation mechanisms~\cite{griewank1989automatic}. 


==> model_linear.tex <==
% Briefly introduce the linearized model. Most readers of this conference would be familiar with the topic, so no need to cover a lot of detail.



Consider a power network with N buses. Let $\bm{V}$ be the voltage vector where $V_i$ is the voltage at bus $i$. Let $\bm{p}$ be active power and $\bm{q}$ be reactive power. The voltage of the system follows the LinDistFlow model in~\cite{zhu2015fast}
\begin{equation}\label{eq:Dyn_voltage}
\bm{V}=\bm{R} \bm{p}+\bm{X} \bm{q}+\mathbbm{1}
\end{equation}
where the reference voltages at each bus is assumed to be 1 p.u., $\mathbbm{1}$ is the all one's vector and $\bm{R}$ and $\bm{X}$ are positive definite matrices defined in~\cite{zhu2015fast}. 


The aim of voltage regulation is to control $\bm{q}$ such that $\bm{V}$ is close to its reference value (e.g., 1 p.u.). 
Due to the lack of communication in many distribution systems, reactive injections need to be successively updated based on the local voltage measurements.


% Due to the lack of communication, $\bm{q}_i$ can only be updated using its local voltage measurement. 
% As local reactive injection affects the whole system, reactive injections need to be successively updated based on the local voltage measurements. 



In this paper we consider linear control updates. Let $k_i$ be the linear control coefficient of the $i$-th bus, and denote $\bm{K} = \operatorname{diag} ( k_{1}, \ldots, k_{N})$. The diagonal matrix $\bm{K}$ means that only local information is used for the control action of each bus.
We update $\bm{q}$ and $\bm{V}$ iteratively as $\bm{q}_{ t+1}=\bm{q}_{t}+\bm{K}(\mathbbm{1} - \bm{V}_{t})$, $\bm{V}_{t+1}=\bm{R} \bm{p}+\bm{X} \left(\bm{q}_{t}+\bm{K}(\mathbbm{1} - \bm{V}_{t}))\right) + \mathbbm{1}$. 

Our objective is to optimize the $k_i$'s to minimize cost subject to the above linear systems in $\bm{V}$ and $\bm{q}$ are stable. 
% The cost function $C(\cdot)$ can be formulated as any convex function such as the $L_1$ or $L_2$ norm on $\bm{V}_t$ and $\bm{q}_t$.
% We obtain an optimal linear coefficient matrix $K$ that guarantees the stability of the system.
The optimization problem is challenging to solve: even with quadratic cost, there is no Algebraic Riccati Equation for diagonal $K$. 
% Many works use learning-based approach to obtain an optimal $K$ through gradient descent. 
% Given that K is diagonal, we cannot solve for optimal K via
% Algebraic Riccati Equation (ARE) and gradient feedback methods require a full-matrix to solve. 
% Therefore we use RL to find an optimal $\bm{K}$.






% We first introduce a discrete time variable t into our equations. 
% The iterative algorithm to update q would be $\bm{q}_{ t+1}=\bm{q}_{t}+\bm{K}(\bm{V}^{ref} - \bm{V}_{t})$ at time t, and denote $\bm{K}$ as $\bm{K}=\operatorname{diag} ( k_{1}, \ldots, k_{n})$, where $k_i$ be the linear coefficient of the $i$-th bus.
% Accordingly, following \eqref{eq:Dyn_voltage}, we update the voltage at time $t+1$ as 



% $\bm{u_t(V_t)}$ is formulated as a static controller that changes reactive power linearly with its local voltage deviation. Let $\alpha_i$ be the linear coefficient of the $i$-th bus and denote $\bm{A}=\operatorname{diag} ( \alpha_{1}, \ldots, \alpha_{n})$. Then the controller is $\bm{u}_t(\bm{V}_t)=\bm{A}\left(\bm{V}^{ref}-\bm{V}_{t}\right)$. 







% Consider a power network $G(\mathcal{N}, \mathcal{E})$ with buses $\mathcal{N} = \{ 0, ..., N\}$. Let $\bm{V}$ be the voltage vector where the $i$-th element is the voltage at the bus $i$. 
% For each line segment ($i$, $j$) between bus $i$ and bus $j$, $r_{ij}$ and $x_{ij}$
% denote its resistance and reactance, respectively. 
% Let $\bm{D}_{r}$ be an $N \times N$ diagonal matrix with the $\ell$ -th diagonal entry equal to $r_{i j}$; and similarly for $\bm{D}_{x}$ which captures all $x_{i j}$ 's.
% Let $\bm{M}$ be the incidence matrix without the reference bus, $\bm{p}$ be active power and $\bm{q}$ be reactive power.
% The voltage of the system follows the LinDistFlow model in~\cite{zhu2015fast}



% \begin{equation}\label{eq:Dyn_voltage}
% \bm{V}=\bm{R} \bm{p}+\bm{X} \bm{q}-\mathbbm{1}
% \end{equation}

% where $\bm{R}:=\bm{M}^{-T} \bm{D}_{r} \bm{M}^{-1}$ and $\bm{X}:=\bm{M}^{-T} \bm{D}_{x} \bm{M}^{-1}$. 



% Voltage regulation is formulated by the following optimization to reduce the total cost: 
% \begin{subequations}\label{eq:Optimization}
% \begin{align}
% \min_{\bm{u}}\quad & \sum_{i=1}^{N} C(\bm{V}_{t}, \bm{q}_t)\label{subeq:Optimization_obj}\\
% \mbox{s.t. } & \bm{q}_{t+1}=\bm{q}_{t}+\bm{u}_t(\bm{V}_t) \label{subeq:Optimization_q}\\
% & \bm{V}_{t+1}=\bm{R} \bm{p}+\bm{X}\left(\bm{q}_{t}+\bm{u}_t(\bm{V}_t)\right)+\mathbbm{1}  \label{subeq:Optimization_V}\\
% & \bm{\underline{u}} \leq \bm{u}_t(\bm{V}_t)\leq \bm{\overline{u}}\label{subeq:Optimization_bound}\\
% &\bm{u}_t(\bm{V}_t) \text{ is stabilizing}\label{subeq:Optimization_stability}
% \end{align}
% \end{subequations}
% where the cost function $C(\cdot)$ can be any convex function such as the $L_1$ or $L_2$ norm on $\bm{V}_t$ and $\bm{q}_t$. The constraint~\eqref{subeq:Optimization_V} represents the changes in reactive power from the controller and~\eqref{subeq:Optimization_q} is the dynamics of voltage from~\eqref{eq:Dyn_voltage}.
% The lower and upper bound for the control action at bus $i$ \highlight{are $\underline{u}_i$ and $\overline{u}_i$, respectively}. Constraints \eqref{subeq:Optimization_q}-\eqref{subeq:Optimization_stability} hold for the time $t$ from 0 to $T$.

% Because of the lack of communication capacity, $\bm{u_t(V_t)}$ is formulated as a static controller that changes reactive power linearly with its local voltage deviation. Let $\alpha_i$ be the linear coefficient of the $i$-th bus and denote $\bm{A}=\operatorname{diag} ( \alpha_{1}, \ldots, \alpha_{n})$. Then the controller is $\bm{u}_t(\bm{V}_t)=\bm{A}\left(\bm{V}^{ref}-\bm{V}_{t}\right)$. We aim to obtain an optimal linear coefficient matrix $A$ from~\eqref{eq:Optimization}. However, \eqref{eq:Optimization} is challenging to solve by conventional control techniques and therefore we use RL to find an optimal $\bm{A}$.


